A Comparison Study of Two Methods for Elliptic Boundary Value Problems

In this paper, we perform a comparison study of two methods (the embedded boundary method and several versions of the mixed finite element method) to solve an elliptic boundary value problem.

==> AComparisonStudy_Scalability.tex <==
     Table \ref{TABLE_SCALABILITY} gives the timing of the methods running in parallel. All grid number are $516\times516$.

\begin{table}
\caption{Scalability}
\label{TABLE_SCALABILITY}          
\begin{tabular}{|c||l|l|l|l|l|}
\hline
num of processors   & time by EBM   & time by RT0   & time by BDM1  & time by RT1   & time by BDM2 \\
1                   & 2.653114      &               &               &               & \\
4                   & 1.293834      &               &               &               & \\
8                   & 0.887960      &               &               &               & \\
16                  & 0.57431       &               &               &               & \\
\hline
\end{tabular}
\end{table}


==> MixedFiniteElementMethod.tex <==

     The mixed finite element method(MFEM) solves the potential $\phi$ and the flux $\nabla\phi$ at the same time. Thus, it solves
\begin{displaymath}    
    \vec{q} = -a\nabla \phi
\end{displaymath}
\begin{displaymath}
    \nabla \cdot \vec{q} = f
\end{displaymath}
For the mixed finite element method, two function spaces are needed: one scalar space for the potential $\phi$ and one vector space for the flux $\vec{q}$. The unknowns are potentials on the elements and flux on the edges. To reduce the problem to a smaller one, the mixed-hybrid finite element is modified by introducing a Lagrangian multiplier on the edges. Chavent and Roberts \cite{Chavent1991} give in detail an implementation using rectangle elements. The final algebraic equations only have TPs (the Lagrangian multiplier, also the potential on the edges) as unknowns, thus reducing the number of unknowns. Later they reduced the problem further by introducing an unknown variable defined inside the element \cite{Chavent1999}. Now instead of unknowns defined on edges, they have only one unknown in each triangle element. Since the number of triangles is much smaller than the number of edges, the problem is reduced into a smaller one. However they only use the lowest order RT basis in their derivation. Since we do not know whether their approach could be extended to use higher order basis functions, our implementation uses the first approach \cite{Chavent1991}. See \cite{BrezziFortin1991} for a more theoretical treatment of the subject.

    In this paper, we use the mixed-hybrid finite element with three different basis functions for flux: the RT0 (Raviart-Thomas space of degree zero), the RT1 (Raviart-Thomas space of degree one) and BDM1(Brezzi-Douglas-Marini space of degree one). 
     The basis function for the flux in RT0 is:
\begin{displaymath}
    \vec{s}|_{K} =    a \left(\begin{array}{l}x\\y\end{array} \right) + \left(\begin{array}{l}b\\c\end{array} \right),
\end{displaymath}
The potential is constant. The lagrangian multiplier TP defined on edges is also constant. RT0 has 1st order accuracy in the flux and potential in $L_2$ norm.

     The basis function for flux in BDM1 is
\begin{displaymath}
    \vec{s}|_{K} =    \left(\begin{array}{l} a_1x+ a_2y+ a_3 \\ b_1x+b_2y+b_3\end{array} \right),
\end{displaymath}
The potential is also constant. However TP is linear. The accuracy for BDM1 is 2rd order in the flux and potential.

     The basis function for the flux in RT1 is
\begin{displaymath}
    \vec{s}|_{K} =    \left(\begin{array}{l} a_1x+ a_2y+ a_3 \\ b_1x+b_2y+b_3\end{array} + \begin{array}{l} x\\ y\end{array} \times (c_1x+c_2y)\right),
\end{displaymath}
and the basis for the potential is a linear function:
\begin{displaymath}
    v|_{K} = P_1 p_1 +P_2 p_2 +P_3 p_3, 
\end{displaymath} 
where $p_1, p_2, p_3$ are the basis function. And TP is also linear. The accuracy is the same as BDM1.

For implementation in details, see \cite{Wang2006, Chavent1991}.


